Data-to-Model Distillation: Data-Efficient Learning Framework

Dataset distillation aims to distill the knowledge of a large-scale real dataset into small yet informative synthetic data such that a model trained on it performs as well as a model trained on the full dataset. Despite recent progress, existing dataset distillation methods often struggle with computational efficiency, scalability to complex high-resolution datasets, and generalizability to deep architectures. These approaches typically require retraining when the distillation ratio changes, as knowledge is embedded in raw pixels. In this paper, we propose a novel framework called Data-to-Model Distillation (D2M) to distill the real dataset's knowledge into the learnable parameters of a pre-trained generative model by aligning rich representations extracted from real and generated images. The learned generative model can then produce informative training images for different distillation ratios and deep architectures. Extensive experiments on 15 datasets of varying resolutions show D2M's superior performance, re-distillation efficiency, and cross-architecture generalizability. Our method effectively scales up to high-resolution 128x128 ImageNet-1K. Furthermore, we verify D2M's practical benefits for downstream applications in neural architecture search.

==> tables/DD_gan.tex <==
 \begin{wraptable}{r}{5.5cm}
  \centering
    \caption{The effect of different generative models on the D2M's performance for the CIFAR10 dataset with IPC1, 10, and 50.}
  \footnotesize
  \setlength{\abovecaptionskip}{0.1cm}
  \resizebox{0.48\textwidth}{!}{
  \begin{tabular}{c|cccc}
    \toprule
    & Conditional GAN  & BigGAN & StyleGAN-XL & CVAE\\
    \midrule
    IPC1 & 49.6±0.7 & 50.2±0.2 & \textbf{50.7±0.5} & 49.8±0.3\\
   IPC10 & 67.4±0.3 & 67.8±0.5 &  \textbf{68.2±0.4} & 67.6±0.2 \\
    IPC50 & 72.2±0.8 & 74.4±0.3 &  \textbf{75.2±0.4} & 73.1±0.4 \\
    
    \bottomrule
  \end{tabular}
   }
    \label{tab:gan}
\end{wraptable} 
